On Rider Strategic Behavior in Ride-Sharing Platforms

Over the past decade, ride-sharing services have become increasingly important, with U.S. market leaders such as Uber and Lyft expanding to over 900 cities worldwide and facilitating billions of rides annually. This rise reflects their ability to meet users' convenience, efficiency, and affordability needs. However, in busy areas and surge zones, the benefits of these platforms can diminish, prompting riders to relocate to cheaper, more convenient locations or seek alternative transportation. While much research has focused on the strategic behavior of drivers, the strategic actions of riders, especially when it comes to riders walking outside of surge zones, remain under-explored. This paper examines the impact of rider-side strategic behavior on surge dynamics. We investigate how riders' actions influence market dynamics, including supply, demand, and pricing. We show significant impacts, such as spillover effects where demand increases in areas adjacent to surge zones and prices surge in nearby areas. Our theoretical insights and experimental results highlight that rider strategic behavior helps redistribute demand, reduce surge prices, and clear demand in a more balanced way across zones.

==> SIG25/model.tex <==
\begin{figure}[!ht]
      \centering
      \includegraphics[width=0.7\textwidth]{fig_final/hexagon_grid.png}
      \caption{The above map schematic represents a geography serviced by a ride-sharing platform. The entire region is divided into hexagonal blocks and the price in each block depends on the market conditions ``locally". Ride-sharing platforms like Uber employ surge pricing algorithms at a ``hyperlocal" level~\cite{uber_pricing}, and Uber in particular uses such hexagonal regions for pricing ~\cite{uber_hex}. The red block represents a region with abnormally high demand, leading to a surge in prices. We call this zone the ``surge zone". In all other surrounding blocks (marked in green), demand reflects usual levels; we call them the ``non-surge zone".}
\end{figure}

We study a model of rider dynamics at surge time on ride-sharing platforms where the riders can be \emph{strategic} and are willing to walk outside of the surge zone to call a ride. This is motivated by behavior observed in practice at large events such as concerts and sports games and backed by empirical research ~\cite{npr}. The paper takes the point of view of the relatively short time horizon that it takes for a surge to happen and clear (minutes to hours). The main goal of the paper is then to understand ride-sharing dynamics over this type of short time scales, with a focus on understanding how demand clears in surge areas during major events. 

To model these dynamics, we study a geography consisting of two main regions: a central region where a major event is happening and where the demand for rides is unusually high, called the \emph{surge zone}; and the surrounding region, initially facing typical demand levels, called the \emph{non-surge zone}. The behavior of drivers (supply side) and riders (demand side) on the platform is formalized below.

\paragraph{Driver's arrivals and behavior:} We consider \emph{non-strategic} drivers that arrive in each zone at an equal, constant, deterministic rate of $\mu$. We \emph{initially} focus on non-strategic drivers to isolate and highlight the role of \emph{rider-side} strategic behavior, which is the main focus of this paper. However, we note that the assumption that rates are equal across zones and that drivers are not strategic, used in the theoretical analysis of Section~\ref{sec:dynamics}, is later relaxed in the experiments of Section~\ref{sec:experiments}. 

\paragraph{Rider's arrivals and behavior:} At time $0$, we consider there is an initial demand in both the surge and the non-surge zone. We denote by $D_{s}(t)$ and $D_{ns}(t)$ the \emph{unmet} demands at the end of time step $t$ in the surge and non-surge zones respectively, and assume throughout the paper that $D_s(0) \gg D_{ns}(0)$. Starting in the first time step, new riders arrive in each zone at a constant, deterministic rate of $\lambda$. We assume\footnote{Otherwise, demand can never be cleared and builds up over time, leading to trivial and uninteresting case.} that $\lambda < \mu$.

Riders can leave each zone via two mechanisms: i) a rider gets matched to a driver and gets a ride; or, ii) a rider can be \emph{strategic} ~\cite{tabloid} (a departure from much of the related work in ride-sharing), and decide \emph{to leave the surge zone in favor of the non-surge zone}, for example when the demand in the surge zone is significantly higher than the demand in the non-surge zone. We make the following assumption on rider behavior in case ii): 

\begin{aspt}\label{as:strat_riders}
The fraction of the unmet rider demand $D_s(t)$ that move from the surge to the non-surge zone at every time step is given by $f \left(D_{s}(t) - D_{ns}(t)\right)$, for a known function $f$. Further, $f(.)$ is non-decreasing, in $[0,1]$, and is positive only if $D_{s}(t) > D_{ns}(t)$.
\end{aspt}

The above condition abstracts away riders' strategic behavior by providing a functional form on the \emph{rate} at which riders decide to move strategically from the surge to the non-surge zone. First, we assume that $f$ is non-decreasing; this is a natural assumption, as the higher the difference in demand and how crowded the surge and non-surge zones are, the more riders are willing to move. Second, we note that the rate is always non-negative: this models the fact that riders would sensibly walk from high-density areas like a stadium or a concert venue to lower-density areas, but not the other way around (e.g., a rider in a busy downtown area walking closer to a major venue or stadium experiencing a surge) may be unrealistic. Second, we note that our functional form makes a \emph{linearity} assumption, where the rate of movement is a function of the difference between demands in the surge and non-surge zones. We provide a motivating explanation of this assumption below:

\begin{example}\label{ex:1}
Assume a simple rider behavior where they make strategic decisions based on price multipliers set by the platform. Denote $m_s(t)$ and $m_{ns}(t)$ respectively the price multipliers in the surge and non-surge zones. Suppose that each agents estimates the price they pay in each zone according to the multipliers, and have a cost $c$ for moving from the surge to non-surge zone. Then the rider's utility for not moving from the surge zone is $m_s(t)$, while the utility for moving is $m_{ns}(t) + c$. In this case, a rider moves if and only if $c \leq m_s(t) - m_{ns}(t)$. When the costs $c$ are i.i.d. from a distribution with c.d.f. F(.), the rate at which riders move is $F(m_s(t) - m_{ns}(t))$. Under a simple pricing rule that is proportional to demand, we recover Assumption~\ref{as:strat_riders}: one such example of a pricing rule could be where the price multiplier depends on the supply-demand mismatch, i.e., $m_s(t) \propto \frac{D_s(t)}{\mu}$ and $m_{ns}(t) \propto \frac{D_{ns}(t)}{\mu}$.

Another motivating explanation is that riders make decision based on \emph{perceived} demand around them. A rider that is in a crowded area perceives that they may be a large demand differential between the surge zone and adjacent, outer areas, and may want to switch locations based on that perceived differential.~~\qedsymbol{}
\end{example}

We note that the assumptions that i) the rate of rider arrivals are deterministic and ii) Assumption~\ref{as:strat_riders} on the specific functional form of riders' behavior, made for the theoretical results of Section~\ref{sec:dynamics}, are relaxed in the experiments of Section~\ref{sec:experiments} in favor of stochastic arrival rates and a game-theoretic model of riders' decisions on which zone to serve as a function of platform prices.




==> SIG25/proofs.tex <==

\subsection{Proof of Theorem \ref{thm:Ds_conv}}\label{app:Ds_conv}
The proof idea is as follows: first, we will show that if $D_s(t)$ reaches $0$ at some time step $t$, it must remain at $0$ for all future time points. Subsequently, if we can show that $D_s(t)$ must reach $0$ in a finite time, this would immediately imply convergence.   

Recall that we have the following update rate for $D_s(t)$:
\[
   D_s(t+1) = \max \left[0, D_s(t) - (\mu - \lambda) - f\left( D_s(t)-D_{ns}(t)\right)\cdot D_s(t) \right].
\]
Since $\mu > \lambda$ (by assumption), $D_s(t) = 0$ implies: 
\[
      D_s(t+1) = \max\left[0, -(\mu-\lambda) \right] = 0.
\]
Now, by induction, we can conclude that $D_s(t+2) = D_s(t+3) = .... = 0$. To complete the rest of the proof, we need to show that starting at $D_s(0) = D_0$, $D_s(t)$ must decrease monotonically to $0$ by at most $\lceil \frac{D_0}{\mu-\lambda} \rceil$ time steps.

Suppose, $D_s(t+1) > 0$. Then, by Eq.~\ref{eq:evolve_s_rev}, we must have:
\begin{align*}
    D_s(t+1) = D_s(t) - (\mu - \lambda) - f \left( D_s(t)-D_{ns}(t) \right)\cdot D_s(t) \leq D_s(t) - (\mu - \lambda).
\end{align*}
The inequality follows because $f(\cdot) \geq 0$ (by definition). 
Thus we have established that $D_s(t)$ is monotonically decreasing until it reaches $0$, where each step (except for the last one) registers a decrease by at least $(\mu-\lambda)$.    
Since $D_s(0) = D_0$, this implies $D_s(t)$ must reach $0$ in atmost $\left \lceil \frac{D_0}{\mu-\lambda} \right \rceil$ steps. This concludes the proof. 


\subsection{Proof of Theorem \ref{thm:Dns_conv}}\label{app:Dns_conv}
We will complete the proof separately for the cases of localized surge and non-localized/spill-over surge. First, we will show in Claim \ref{clm:local_surge} that under the condition for a localized surge, $D_{ns}(t)$ is monotonically decreasing until it reaches $0$ and then it stays at $0$ for all future time points. 

\begin{claim}\label{clm:local_surge}
When $D_0 \cdot f\left(D_0-d_0 \right) \leq \mu - \lambda$, $D_{ns}(t)$ is non-increasing for all $t \in \{0, 1, 2,....\}$ and it converges to $0$ in finite time.  
\end{claim}
\begin{proof}
The proof is by induction. We know that $D_{ns}(0) = 0$.\jz{should not be here anymore} \\ \\
\emph{Base Case ($D_{ns}(1) = 0$)\jz{issue with the base case here too}: } From Eq~\eqref{eq:evolve_ns_rev}, we have: 
\[
   D_{ns}(1) = \max \left[0, (\lambda - \mu) + f\left(D_0 \right)\cdot D_0 \right] = 0,
\]
where the last equality follows because $D_0 \cdot f\left(D_0 \right) \leq \mu - \lambda$. \\ \\
\emph{Induction Hypothesis:} Suppose, we have $D_{ns}(t) = 0$ for some $t > 1$. \\
\emph{General Case:} Now, if we can show that $D_{ns}(t+1) = 0$, we are done. 
\begin{align*}
    D_{ns}(t+1) &= \max \left[0, D_{ns}(t) + (\lambda-\mu) + f\left(D_s(t)-D_{ns}(t) \right)\cdot D_s(t) \right] \\
    &= \max \left[0, (\lambda - \mu) + f\left( D_s(t) \right)\cdot D_s(t) \right] \\
    &\leq \max \left[0, (\lambda - \mu) + f\left( D_0 \right)\cdot D_0 \right] \\ 
    &= 0.
\end{align*}
The first equality results from using the induction hypothesis $D_{ns}(t) = 0$. The inequality follows because $D_s(t)$ is non-increasing (by Theorem \ref{thm:Ds_conv}) and $f(\cdot)$ is non-decreasing in its argument. Finally, the last step follows from the localized surge condition. This concludes the proof. 
\end{proof}

When the surge is not localized, i.e., $D_0 \cdot f\left(D_0 \right) > \mu - \lambda$, our first goal is to prove convergence of $D_{ns}(t)$. We show this in Claim \ref{clm:total_unmet_dec}. The proof uses the fact that $D_s(t)$ is guaranteed to converge in finite time. Then subsequently, we argue about the shape of $D_{ns}(t)$ in Lemma \ref{lem:tau_exist} to complete the proof of the theorem.

\begin{claim}\label{clm:total_unmet_dec}
When $D_0 \cdot f\left(D_0 \right) > \mu - \lambda$, the waiting demand outside the surge zone at the end of time step $t$, given by $D_{ns}(t)$, converges to $0$ in finite time. 
\end{claim}
\begin{proof}
We have already established in the proof of Theorem \ref{thm:Ds_conv} that $D_s(t)$ goes to $0$ in atmost $\lceil \frac{D_0}{\mu-\lambda} \rceil$ time steps and remains there for all future time steps. Define $t' := \lceil \frac{D_0}{\mu-\lambda} \rceil$. Now, there are two cases: 
\paragraph{Case 1 ($D_{ns}(t') = 0$):} From Eq.~\eqref{eq:evolve_ns_rev}, we obtain: 
\begin{align*}
    D_{ns}(t'+1) = \max \left[0, (\lambda - \mu) \right] = 0. 
\end{align*}
This follows directly because $D_s(t') = 0$ and $\lambda < \mu$. By induction, we conclude that $D_{ns}(t) = 0$ for all $t > t'$ and hence, we have convergence.

\paragraph{Case 2 ($D_{ns}(t') > 0$):} We know that $D_s(t) = 0$ for all $t \geq t'$. Therefore,
\begin{align*}
    D_{ns}(t'+1) = \max \left[0, D_{ns}(t') - (\mu-\lambda) \right] = \begin{cases}
     D_{ns}(t') - (\mu - \lambda), \quad if~D_{ns}(t') > \mu-\lambda,\\
     0, \quad o/w.
    \end{cases}
\end{align*}
We can extend the above argument to show that for any $t >  t'$, 
\[
   D_{ns}(t) = \max \left[0, D_{ns}(t') - (t-t')(\mu - \lambda) \right].
\]
Thus $D_{ns}(t)$ must reach $0$ in at most $\frac{D_{ns}(t')}{\mu - \lambda}$ additional steps beyond $t'$. Following this, Case 1 indicates that $D_{ns}(t)$ must stay at $0$ for all later time points and hence, the convergence result follows.
\end{proof}

Finally, we want to understand how $D_{ns}(t)$ behaves in the short term. We show that $D_{ns}(t)$ has a single peak attained at some time point $\tau$ beyond which it decreases monotonically to $0$. Formally, we present Lemma~\ref{lem:tau_exist}. 

\begin{lemma}\label{lem:tau_exist}
Suppose, $D_0$ satisfies $D_0 \cdot f\left(D_0 \right) > \mu - \lambda$. Then, there exists some time step $\tau > 0$ such that $D_{ns}(t)$ is monotonically increasing until $\tau$ and non-increasing beyond $\tau$. $\tau$ is given by: 
\[
       \tau = \min \{t: f \left( D_s(t)-D_{ns}(t) \right) \cdot D_s(t) \leq (\mu - \lambda)\}.
\]
\end{lemma}
\begin{proof}
The proof is divided into two parts: in the first part, we will argue why $D_{ns}(t)$ must increase monotonically for all $t \leq \tau$. Then, in the second part, we will show that it must be non-increasing for all $t > \tau$. \\

First, note that $f\left(D_0\right)\cdot D_0 > \mu - \lambda$. Hence from definition, $\tau \geq 1$ and it is also clear that for all $t < \tau$, 
\[
      f \left( D_s(t)-D_{ns}(t) \right) \cdot D_s(t) > (\mu - \lambda). 
\]
This implies that for all $t < \tau$, if $D_{ns}(t) \geq 0$,
\begin{align*}
    D_{ns}(t+1) &= \max \left[ 0, D_{ns}(t) + (\lambda - \mu) + f \left( D_s(t)-D_{ns}(t) \right) \cdot D_s(t)\right]
    >  D_{ns}(t). 
\end{align*}
Thus, we have $D_{ns}(\tau) > D_{ns}(\tau-1) > .... D_{ns}(1) > D_{ns}(0) = 0$. This concludes part one of the proof. 

For part two, we need to prove that $D_{ns}(t)$ is always non-increasing beyond $\tau$. Actually, it suffices to show that:
\begin{align}\label{temp}
    f \left( D_s(t)-D_{ns}(t) \right)\cdot D_s(t) \leq (\mu - \lambda) \quad \forall ~t \geq \tau.
\end{align}
We will do a proof by induction: \\
\emph{Base Case: }From the definition of $\tau$, we already know that \eqref{temp} holds at $t = \tau$. This implies $D_{ns}(\tau+1) \leq D_{ns}(\tau)$. \\
\emph{Induction Hypothesis:} Suppose, \eqref{temp} holds for some $t' > \tau$.\\
\emph{General Case: } We now need to show that \eqref{temp} also holds for $t'+1$. There are two cases to be considered:
\begin{itemize}
    \item Suppose, $D_s(t') = 0$. In that case, by Theorem~\ref{thm:Ds_conv}, $D_s(t'+1) = 0$. This implies:
    \[
          f \left( D_s(t'+1)-D_{ns}(t'+1) \right)\cdot D_s(t'+1) = 0 \leq (\mu - \lambda).
    \]
    \item Now, suppose, $D_s(t') > 0$. If $D_s(t'+1) = 0$, we are done again (trivially). If not, i.e., $D_s(t'+1) > 0$, we have:
    \begin{align*}
        &D_s(t'+1) - D_{ns}(t'+1)\\
        = &D_s(t') + (\lambda - \mu) - f\left( D_s(t')-D_{ns}(t') \right) \cdot D_s(t') \\
        & \quad - \max \left[0, D_{ns}(t') + (\lambda-\mu) + f\left( D_s(t')-D_{ns}(t')\right)\cdot D_s(t') \right] \\
        \leq & D_s(t') + (\lambda - \mu) - f\left( D_s(t')-D_{ns}(t') \right) \cdot D_s(t') \\
        &\quad - \left( D_{ns}(t') + (\lambda-\mu) + f\left( D_s(t')-D_{ns}(t')\right)\cdot D_s(t') \right)\\
        = & D_s(t') - D_{ns}(t') - f\left( D_s(t')-D_{ns}(t')\right)\cdot D_s(t') \\
        \leq & D_s(t') - D_{ns}(t').
    \end{align*}
\end{itemize}
The first step follows because $D_s(t'+1) > 0$ by assumption. The inequality in the second step results from the observation that removing the $\max(\cdot)$ can only increase the difference, with exact equality holding if $D_{ns}(t'+1) > 0$. The last step follows since $f(\cdot) \geq 0$ and $D_s(t') \geq 0$. Therefore, by the non-decreasing property of $f(\cdot)$, we must have:
\[
   f\left( D_s(t'+1) - D_{ns}(t'+1) \right) \leq f \left( D_s(t') - D_{ns}(t') \right)
\]
Finally, since $D_s(t'+1) \leq D_s(t')$ by Theorem~\ref{thm:Ds_conv}, we establish the desired inequality and conclude the proof.
\[
   f\left( D_s(t'+1) - D_{ns}(t'+1) \right) \cdot D_s(t'+1) \leq f \left( D_s(t') - D_{ns}(t') \right)\cdot D_s(t') \leq \mu - \lambda. 
\]
\end{proof}

\subsection{Proof of Theorem \ref{thm:bounds_Ds}}\label{app:bounds_conv}
We will complete the proof in two parts: first we will establish the bounds for the localized surge case in Lemma \ref{lem:bounds_convergence_local} followed by the non-localized surge case in Lemma \ref{lem:bounds_convergence_n}. Combining both lemmas, we have the proof of the theorem. 

\begin{lemma}\label{lem:bounds_convergence_local}
The time to convergence for $D_s(t)$ in the localized surge setting, given by $\tau_s^{loc}$, must satisfy: 
\[
         \left\lfloor \frac{D_0}{2(\mu - \lambda)} \right\rfloor  \leq \tau_s^{loc} \leq \left\lceil \frac{D_0}{(\mu - \lambda)} \right\rceil.
\]
\end{lemma}
\begin{proof}
We have already established in the proof of Theorem~\ref{thm:Ds_conv} that $\tau_s \leq \lceil \frac{D_0}{(\mu - \lambda)} \rceil$. We need to establish the lower bound now.
Observe that $D_s(t)$ decays to $0$ faster in the \textit{localized surge} setting. This is because, $D_{ns}(t)$ is always equal to $0$ in localized surge, so the demand gradient across the surge boundary is larger which leads to faster decay. 

Recall, in localized surge, we have the following equation for evolution of $D_s(t)$ over time:
\[
   D_s(t+1) = \max\left[0, D_s(t) - (\mu - \lambda) - f\left( D_s(t)\right)\cdot D_s(t) \right].
\]
Since $D_s(0) = D_0 > 0$ and we are interested in the time to convergence to $0$, given by $\tau_s^{loc}$, we can drop the maximum operator. Therefore, the revised update rule of $D_s(t)$ is as follows: 
\[
   D_s(t+1) = D_s(t) - (\mu - \lambda) - f\left( D_s(t)\right)\cdot D_s(t). 
\]
Using the structure of the update rule, we adopt a telescopic sum approach: 
\begin{align*}
    D_s(\tau_s^{loc}) - D_s(\tau_s^{loc}-1) &= - (\mu - \lambda) - f\left(D_s(\tau_s^{loc}-1) \right) \cdot D_s(\tau_s^{loc}-1) \\
    &......\\
    D_s(1) - D_s(0) &= - (\mu - \lambda) - f\left(D_s(0) \right) \cdot D_s(0).
\end{align*}
Adding up all equations, we obtain: 
\[
    D_s(\tau_s^{loc}) - D_s(0) = -\tau_s^{loc}(\mu - \lambda) - \sum_{t=0}^{\tau_s^{loc}-1} f\left(D_s(t) \right) \cdot D_s(t)
\]
By assumption, $D_s(\tau_s^{loc}) = 0$. Also, we know that $D_s(0) = D_0$. Therefore, the above equation is equivalent to:
\begin{align*}
   D_0 &= \tau_s^{loc} (\mu - \lambda) + \sum_{t=0}^{\tau_s^{loc}-1} f\left(D_s(t) \right) \cdot D_s(t) \\
   &\leq  \tau_s^{loc} (\mu - \lambda) + \tau_s^{loc} f\left( D_0 \right)\cdot D_0 \\
   & \leq 2 \tau_s^{loc} (\mu - \lambda). 
\end{align*}
The first inequality follows because $D_s(t)$ is non-increasing (Refer Theorem~\ref{thm:Ds_conv}) and $f(\cdot)$ is increasing in its argument (by assumption). The last step follows from the \textit{localized surge} condition. Therefore, we have the desired lower bound on $\tau_s^{loc}$: 
\[
      \tau_s^{loc} \geq \frac{D_0}{2(\mu - \lambda)} \geq \left\lfloor \frac{D_0}{2(\mu - \lambda)} \right\rfloor. 
\]
\end{proof}

\begin{lemma}\label{lem:bounds_convergence_n}
The time to convergence for $D_s(t)$ in the non-localized surge setting, given by $\tau_s^{n}$, must satisfy: 
\[
         \left\lfloor \frac{D_0}{(\mu - \lambda) + D_0 \cdot f(D_0/\mu)} \right\rfloor  \leq \tau_s^{n} \leq \left\lceil \frac{D_0}{(\mu - \lambda)} \right\rceil.
\]
\end{lemma}
% \jz{it's a bit weird compared to lemma 2. In lemma 2 you bound both terms in the denominator by the max of them, You probably should do the same here?}\ds{you're right, but the D0 term can be very very large, in which case, replacing it by 2 $\times$ D0 term would make the lower bound very loose}
\begin{proof}
The proof idea is similar to Lemma \ref{lem:bounds_convergence_local}. The update rule for $D_s(t)$ is given by: 
\begin{align*}
    D_s(t+1) &= D_s(t) - (\mu - \lambda) - f\left( D_s(t)-D_{ns}(t) \right)\cdot D_s(t) \\
    &\geq D_s(t) - (\mu - \lambda) - f\left( D_s(t) \right)\cdot D_s(t)
\end{align*}
The inequality follows because $D_s(t) - D_{ns}(t) \leq D_s(t)$ and $f(\cdot)$ is non-decreasing in its argument by definition. Using a telescopic sum approach like earlier, we obtain: 
\[
     D_s(\tau^n) - D_0 \geq -\tau_s^n(\mu - \lambda) - \sum_{t=0}^{\tau_s^n-1}f\left( D_s(t) \right)\cdot D_s(t).
\]
Plugging $D_s(\tau^n) = 0$ and flipping the inequality (due to the negative sign), we have:
\[
     D_0 \leq \tau_s^n(\mu - \lambda) + \sum_{t=0}^{\tau_s^n-1}f\left( D_s(t) \right)\cdot D_s(t) \leq \tau_s^n(\mu - \lambda) + \tau_s^n f\left( D_0\right)\cdot D_0
\]
This results in the desired lower bound on $\tau_s^n$:
\[
    \tau_s^n \geq \frac{D_0}{(\mu - \lambda) + D_0 \cdot f(D_0)} \geq \left \lfloor \frac{D_0}{(\mu - \lambda) + D_0 \cdot f(D_0)} \right\rfloor.
\]
\end{proof}


